IMBERT: Making BERT Immune to Insertion-based Backdoor Attacks

Backdoor attacks are an insidious security threat against machine learning models. Adversaries can manipulate the predictions of compromised models by inserting triggers into the training phase. Various backdoor attacks have been devised which can achieve nearly perfect attack success without affecting model predictions for clean inputs. Means of mitigating such vulnerabilities are underdeveloped, especially in natural language processing. To fill this gap, we introduce IMBERT, which uses either gradients or self-attention scores derived from victim models to self-defend against backdoor attacks at inference time. Our empirical studies demonstrate that IMBERT can effectively identify up to 98.5% of inserted triggers. Thus, it significantly reduces the attack success rate while attaining competitive accuracy on the clean dataset across widespread insertion-based attacks compared to two baselines. Finally, we show that our approach is model-agnostic, and can be easily ported to several pre-trained transformer models.

==> algo_grad.tex <==
\renewcommand{\algorithmiccomment}[1]{\hfill\eqparbox{ }{$\triangleright$ #1}}
% \algnewcommand{\LineComment}[1]{\STATE \(\triangleright\) #1}
\begin{algorithm}[t] % enter the algorithm environment
\caption{DelToken($\vx, \vm, \mI$)} % give the algorithm a caption
\label{alg:del} % and a label for \ref{} commands later in the document
\begin{algorithmic}[1] % enter the algorithmic environment
\REQUIRE input sentence $\vx$, mask $\vm$, a set of indices $\mI$
\ENSURE processed input $\vx'$,  processed mask $\vm'$
         \STATE {$\vx' \leftarrow \{\}$}
         \STATE {$\vm' \leftarrow \{\}$}
         \FOR{$i$ in range($|\vx|$)}
         \IF{$i \not\in \mI_k$}
         \STATE {$\vx' \leftarrow \vx'\bigcup \vx[i]$}
         \STATE {$\vm' \leftarrow \vm'\bigcup \vm[i]$}
         \ENDIF
         \ENDFOR
         
         \RETURN $\vx'$, $\vm'$
\end{algorithmic}
\end{algorithm}

==> algo_mask.tex <==
\renewcommand{\algorithmiccomment}[1]{\hfill\eqparbox{ }{$\triangleright$ #1}}
% \algnewcommand{\LineComment}[1]{\STATE \(\triangleright\) #1}
\begin{algorithm}[t] % enter the algorithm environment
\caption{MaskToken($\vx, \vm, \mI$)} % give the algorithm a caption
\label{alg:mask} % and a label for \ref{} commands later in the document
\begin{algorithmic}[1] % enter the algorithmic environment
\REQUIRE input sentence $\vx$, mask $\vm$, a set of indices $\mI$
\ENSURE processed input $\vx'$,  processed mask $\vm'$
         \STATE {$\vx' \leftarrow \{\}$}
         \STATE {$\vm' \leftarrow \{\}$}
         \FOR{$i$ in range($|\vx|$)}
         \STATE {$\vx' \leftarrow \vx'\bigcup \vx[i]$}
         \IF{$i \in \mI_k$}
         \STATE {$\vm[i] \leftarrow 0$}
         \ENDIF
          \STATE {$\vm' \leftarrow \vm'\bigcup \vm[i]$}
         \ENDFOR
         
         \RETURN $\vx'$, $\vm'$
\end{algorithmic}
\end{algorithm}

==> tab_r1.tex <==
\begin{table*}[]
    \centering
    
    \begin{tabular}{p{0.95\linewidth}}
    \toprule
         \textbf{Reviewer 1} \\
        \midrule
        \textbf{What is this paper about and what contributions does it make?}\\
\midrule
This paper is about protecting BERT from insertion-based Backdoor Attacks. Two methods are described and investigated experimentally against two baselines.\\
\midrule


\textbf{Reasons to accept}\\
\midrule
Their method significantly outperforms the two chosen baselines for insertion-based backdoor attacks\\
\midrule


\textbf{Reasons to reject}\\
\midrule
There seems to be no good way to choose the hyperparameters, e.g., K, in Algorithm 1.\\

The backdoor attacks seems too simple to defend against. It seems that they can also be easily detected by humans.
 It is not clear whether the authors tried some simpler techniques first, before coming up with these two methods.

It seems that mitigating such backdoor attacks may not be sufficient to protect models anyway. For example, see Goldwasser et al. "Planting Undetectable Backdoors in Machine Learning Models" in IEEE FOCS 2022\\
\midrule


\textbf{Questions for the Author(s)}\\
\midrule
Question A: What about the performance of your methods if the model was trained with a loss function that is not known to you? Did you check the performance of your methods in such a scenario?\\
\midrule


\textbf{Missing References}\\
\midrule
1) Is this paper on Arxiv related? Defending Against Stealthy Backdoor Attacks
Sangeet Sagar, Abhinav Bhatt, Abhijith Srinivas Bidaralli\\

2) Goldwasser et al. "Planting Undetectable Backdoors in Machine Learning Models" in IEEE FOCS 2022\\
\midrule


\textbf{Typos, Grammar, Style, and Presentation Improvements}\\
\midrule
Figures 2 and 3 are so too small to convey any  useful information\\
\midrule

\textbf{Reviewer's Scores}\\
\midrule
                               Soundness: 3\\
                 Excitement (Long paper): 2.5\\
                     Reviewer Confidence: 4\\
     Recommendation for Best Paper Award: No\\
                         Reproducibility: 3\\
                        Ethical Concerns: No\\


\bottomrule
    \end{tabular}
    \caption{Comments of Reviewer 1.}
    \label{tab:r1}
\end{table*}

\begin{table*}[]
    \centering
    
    \begin{tabular}{p{0.95\linewidth}}
    \toprule
         \textbf{Reviewer 2} \\
        \midrule
        \textbf{What is this paper about and what contributions does it make?}\\
\midrule
This paper introduces IMBERT which uses either gradients or self-attention scores to self-defend against backdoor attacks at inference time. Specifically, the proposed approach leverages gradients and self-attention scores to locate triggers and then remove or mask triggers before making prediction. The paper evaluates the proposed approach against four backdoor attacks on three text classification tasks.\\
\midrule


\textbf{Reasons to accept}\\
\midrule
(1) Simple but efficient idea. The proposed idea may provide insights into investigation of defense solution against backdoor attacks. \\

(2) Sufficient experiments in text classification for evaluation. Specifically, the paper evaluates the proposed approach against four backdoor attacks (BadNet, RIPPLES, InsertSent, Syntactic) on three text classification tasks (SST-2, OLID, AG News). The analysis is also comprehensive.
\\
\midrule


\textbf{Reasons to reject}\\
\midrule
1) Analysis of gradient distribution and rationale of having a threshold are unclear. According to my understanding (also the related work by Wallace et al. (2019)), the larger magnitude of the gradient, the more importance of the token in making decision. In Table 2, the IMBERT-G identifies more than 94\% triggers for BadNet. This result also indicates that most of triggers have larger gradients. However, it contradicts to the observation of Figure 2(a). In addition, L2 norm of the partial derivative is not defined clearly.\\
\midrule


\textbf{Questions for the Author(s)}\\
\midrule
Question A: The gradient approach aims to seek the triggers through the gradients of the input tokens. Table 2 also indicates that most of triggers have larger gradients (more than 94\% triggers are identifies using top K selection method). However, why the gradient distribution in Figure 2(a) shows that most of triggers have small gradients? When including a threshold for gradient, what would be the results in Table 2? In other words, will including a threshold for gradient increase or decrease TopK precision?\\
\midrule

\textbf{Reviewer's Scores}\\
\midrule
                                                 Soundness: 3\\
                 Excitement (Long paper): 3.5\\
                     Reviewer Confidence: 4\\
     Recommendation for Best Paper Award: No\\
                         Reproducibility: 5\\
                        Ethical Concerns: No\\



\bottomrule
    \end{tabular}
    \caption{Comments of Reviewer 2.}
    \label{tab:r2}
\end{table*}

\begin{table*}[]
    \centering
    
    \begin{tabular}{p{0.95\linewidth}}
    \toprule
         \textbf{Reviewer 3} \\
        \midrule
        \textbf{What is this paper about and what contributions does it make?}\\
\midrule
The paper presents a defense approach against insertion-based backdoor attacks for pre-trained model BERT. The core idea is to use gradients or self-attention scores to identify tokens with the most significant influence and mask them to make the model robust. With experiments on three datasets and four potential attack methods, the author proves the effectiveness of the method on insertion-based attack types and also shows the performance drop is within the reasonable range.\\
\midrule


\textbf{Reasons to accept}\\
\midrule
+ Important question, intuitive approach with reasonable implementation \\
+ Comprehensive discussion of different attacks and related experiments \\
+ Insightful reasoning about trigger identification and poisoning illustration \\
\midrule


\textbf{Reasons to reject}\\
\midrule
- Lack of reasoning about the value selection of K and lambda, not sure if it is generally applicable to other datasets \\
- Questionable comparison with previous work, especially the performance comparison with ONION for the BadNet attack\\
- Lack of discussion on attacks that "directly adjust the weights” indeed losses generality \\
\midrule


\textbf{Questions for the Author(s)}\\
\midrule
Question A: In comparison with ONION (Qi et al., 2021a), I cannot find the experiment numbers that are reported in this paper. Did I miss something? Or is the setting different?\\
\midrule

\textbf{Reviewer's Scores}\\
\midrule
                             Soundness: 2\\
                 Excitement (Long paper): 2.5\\
                     Reviewer Confidence: 3\\
     Recommendation for Best Paper Award: No\\
                         Reproducibility: N/A\\
                        Ethical Concerns: No\\

\bottomrule
    \end{tabular}
    \caption{Comments of Reviewer 3.}
    \label{tab:r3}
\end{table*}
